HFODD (v2.40h) User's Guide

We describe the input data and installation procedures of the code HFODD (v2.40h). The present write-up contains complete and comprehensive information that has originally been given in six independent publications. It is enhanced by the subject index and indexes of variables, input-data keywords, subroutines, and files that are used in this user guide.

==> index_of_files.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item {\textcolor{magenta}    {{\tt{dy152-a.dat}}}}, 73, 74
  \item {\textcolor{magenta}    {{\tt{dy152-a.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152-b.dat}}}}, 73, 74
  \item {\textcolor{magenta}    {{\tt{dy152-b.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152-c.dat}}}}, 73, 74
  \item {\textcolor{magenta}    {{\tt{dy152-c.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152-d.dat}}}}, 73, 74
  \item {\textcolor{magenta}    {{\tt{dy152-d.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152-e.dat}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152-e.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152-f.dat}}}}, 73, 74
  \item {\textcolor{magenta}    {{\tt{dy152-f.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{dy152e-dat}}}}, 74
  \item {\textcolor{magenta}    {{\tt{dy152f-dat}}}}, 74

  \indexspace

  \item {\textcolor{magenta}    {{\tt{ge064-a.dat}}}}, 73, 79
  \item {\textcolor{magenta}    {{\tt{ge064-a.out}}}}, 68, 73
  \item {\textcolor{magenta}    {{\tt{ge064-b.dat}}}}, 73, 79, 80
  \item {\textcolor{magenta}    {{\tt{ge064-b.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{ge064-c.dat}}}}, 73, 80

  \indexspace

  \item {\textcolor{magenta}    {{\tt{hfodd.f}}}}, 69, 70, 72

  \indexspace

  \item {\textcolor{magenta}    {{\tt{la132-a.dat}}}}, 73, 76, 78
  \item {\textcolor{magenta}    {{\tt{la132-a.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{la132-b.dat}}}}, 73, 76, 78
  \item {\textcolor{magenta}    {{\tt{la132-b.out}}}}, 73

  \indexspace

  \item {\textcolor{magenta}    {{\tt{pb128-a.dat}}}}, 73
  \item {\textcolor{magenta}    {{\tt{pb208-a.dat}}}}, 78
  \item {\textcolor{magenta}    {{\tt{pb208-a.out}}}}, 73

  \indexspace

  \item {\textcolor{magenta}    {{\tt{sn120-a.dat}}}}, 73, 79
  \item {\textcolor{magenta}    {{\tt{sn120-a.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{sn120-b.dat}}}}, 73, 80
  \item {\textcolor{magenta}    {{\tt{sn120-b.out}}}}, 73

  \indexspace

  \item {\textcolor{magenta}    {{\tt{tb-151-d.dat}}}}, 76
  \item {\textcolor{magenta}    {{\tt{tb151-a.dat}}}}, 73, 75, 76
  \item {\textcolor{magenta}    {{\tt{tb151-a.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{tb151-b.dat}}}}, 73, 76
  \item {\textcolor{magenta}    {{\tt{tb151-b.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{tb151-c.dat}}}}, 73, 76
  \item {\textcolor{magenta}    {{\tt{tb151-c.out}}}}, 73
  \item {\textcolor{magenta}    {{\tt{tb151-d.dat}}}}, 73, 75
  \item {\textcolor{magenta}    {{\tt{tb151-d.out}}}}, 73

\end{theindex}


==> index_of_keywords.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item {\textcolor{blue}    {{\tt{ALL\_DONE}}}}, 8

  \indexspace

  \item {\textcolor{blue}    {{\tt{BASIS\_SIZE}}}}, 48, 69
  \item {\textcolor{blue}    {{\tt{BCS}}}}, 28
  \item {\textcolor{blue}    {{\tt{BLOCKFIX\_N}}}}, 44
  \item {\textcolor{blue}    {{\tt{BLOCKFIX\_P}}}}, 44
  \item {\textcolor{blue}    {{\tt{BLOCKSIG\_N}}}}, 42
  \item {\textcolor{blue}    {{\tt{BLOCKSIG\_P}}}}, 43
  \item {\textcolor{blue}    {{\tt{BLOCKSIM\_N}}}}, 37
  \item {\textcolor{blue}    {{\tt{BLOCKSIM\_P}}}}, 37
  \item {\textcolor{blue}    {{\tt{BLOCKSIQ\_N}}}}, 40
  \item {\textcolor{blue}    {{\tt{BLOCKSIQ\_P}}}}, 40
  \item {\textcolor{blue}    {{\tt{BLOCKSIZ\_N}}}}, 34
  \item {\textcolor{blue}    {{\tt{BLOCKSIZ\_P}}}}, 35
  \item {\textcolor{blue}    {{\tt{BOHR\_BETAS}}}}, 54
  \item {\textcolor{blue}    {{\tt{BROYDEN}}}}, 46

  \indexspace

  \item {\textcolor{blue}    {{\tt{CHAOTIC}}}}, 12
  \item {\textcolor{blue}    {{\tt{CHECKERNEL}}}}, 31
  \item {\textcolor{blue}    {{\tt{CONT\_OMEGA}}}}, 63
  \item {\textcolor{blue}    {{\tt{CONT\_PAIRI}}}}, 63
  \item {\textcolor{blue}    {{\tt{CONTFIELDS}}}}, 22, 64
  \item {\textcolor{blue}    {{\tt{CONTLIPKIN}}}}, 64
  \item {\textcolor{blue}    {{\tt{CONTYUKAWA}}}}, 64
  \item {\textcolor{blue}    {{\tt{COULOMB}}}}, 45
  \item {\textcolor{blue}    {{\tt{COULOMBPAR}}}}, 22
  \item {\textcolor{blue}    {{\tt{COULOMFILE}}}}, 59
  \item {\textcolor{blue}    {{\tt{COULOMSAVE}}}}, 59
  \item {\textcolor{blue}    {{\tt{CUTOFF}}}}, 21
  \item {\textcolor{blue}    {{\tt{CUTOVERLAP}}}}, 32

  \indexspace

  \item {\textcolor{blue}    {{\tt{DIANON\_NEU}}}}, 34
  \item {\textcolor{blue}    {{\tt{DIANON\_PRO}}}}, 34
  \item {\textcolor{blue}    {{\tt{DIAPAR\_NEU}}}}, 34, 39
  \item {\textcolor{blue}    {{\tt{DIAPAR\_PRO}}}}, 40
  \item {\textcolor{blue}    {{\tt{DIASIG\_NEU}}}}, 42
  \item {\textcolor{blue}    {{\tt{DIASIG\_PRO}}}}, 42
  \item {\textcolor{blue}    {{\tt{DIASIM\_NEU}}}}, 37
  \item {\textcolor{blue}    {{\tt{DIASIM\_PRO}}}}, 37

  \indexspace

  \item {\textcolor{blue}    {{\tt{EALLMINMAX}}}}, 55
  \item {\textcolor{blue}    {{\tt{EPS\_HERMIT}}}}, 46
  \item {\textcolor{blue}    {{\tt{EQUASI\_MAX}}}}, 55
  \item {\textcolor{blue}    {{\tt{EVE\_ADD\_PM}}}}, 18
  \item {\textcolor{blue}    {{\tt{EVE\_ADD\_TS}}}}, 18
  \item {\textcolor{blue}    {{\tt{EVE\_SCA\_PM}}}}, 17
  \item {\textcolor{blue}    {{\tt{EVE\_SCA\_TS}}}}, 16, 18, 66
  \item {\textcolor{blue}    {{\tt{EXECUTE}}}}, 8, 9, 58, 73, 74

  \indexspace

  \item {\textcolor{blue}    {{\tt{FIELD\_OLD}}}}, 62
  \item {\textcolor{blue}    {{\tt{FIELD\_SAVE}}}}, 23, 62
  \item {\textcolor{blue}    {{\tt{FILSIG\_NEU}}}}, 28
  \item {\textcolor{blue}    {{\tt{FILSIG\_PRO}}}}, 29
  \item {\textcolor{blue}    {{\tt{FIXDELTA\_N}}}}, 20
  \item {\textcolor{blue}    {{\tt{FIXDELTA\_P}}}}, 20
  \item {\textcolor{blue}    {{\tt{FIXFERMI\_N}}}}, 33
  \item {\textcolor{blue}    {{\tt{FIXFERMI\_P}}}}, 33
  \item {\textcolor{blue}    {{\tt{FIXLAMB2\_N}}}}, 32
  \item {\textcolor{blue}    {{\tt{FIXLAMB2\_P}}}}, 32

  \indexspace

  \item {\textcolor{blue}    {{\tt{G\_SCALING}}}}, 19
  \item {\textcolor{blue}    {{\tt{GAUSHERMIT}}}}, 46, 69

  \indexspace

  \item {\textcolor{blue}    {{\tt{HBAR2OVR2M}}}}, 15
  \item {\textcolor{blue}    {{\tt{HFB}}}}, 28
  \item {\textcolor{blue}    {{\tt{HFBMEANFLD}}}}, 56
  \item {\textcolor{blue}    {{\tt{HOMEGAZERO}}}}, 48

  \indexspace

  \item {\textcolor{blue}    {{\tt{INI\_DELTA}}}}, 19
  \item {\textcolor{blue}    {{\tt{INI\_FERMI}}}}, 19
  \item {\textcolor{blue}    {{\tt{INI\_INVERS}}}}, 29
  \item {\textcolor{blue}    {{\tt{INI\_LIPKIN}}}}, 32
  \item {\textcolor{blue}    {{\tt{INI\_ROTAT}}}}, 29
  \item {\textcolor{blue}    {{\tt{INSERT\_HO}}}}, 24
  \item {\textcolor{blue}    {{\tt{ITERAT\_EPS}}}}, 10
  \item {\textcolor{blue}    {{\tt{ITERATIONS}}}}, 10

  \indexspace

  \item {\textcolor{blue}    {{\tt{KERNELFILE}}}}, 60

  \indexspace

  \item {\textcolor{blue}    {{\tt{LANDAU}}}}, 15
  \item {\textcolor{blue}    {{\tt{LANDAU-SAT}}}}, 16
  \item {\textcolor{blue}    {{\tt{LIPKIN}}}}, 32
  \item {\textcolor{blue}    {{\tt{LIPKINSAVE}}}}, 61

  \indexspace

  \item {\textcolor{blue}    {{\tt{MAX\_MAGNET}}}}, 45
  \item {\textcolor{blue}    {{\tt{MAX\_MULTIP}}}}, 45
  \item {\textcolor{blue}    {{\tt{MAX\_SURFAC}}}}, 45
  \item {\textcolor{blue}    {{\tt{MAXANTIOSC}}}}, 10
  \item {\textcolor{blue}    {{\tt{MULTCONSCA}}}}, 54
  \item {\textcolor{blue}    {{\tt{MULTCONSTR}}}}, 53

  \indexspace

  \item {\textcolor{blue}    {{\tt{NILSSONLAB}}}}, 57
  \item {\textcolor{blue}    {{\tt{NILSSONPAR}}}}, 64
  \item {\textcolor{blue}    {{\tt{NORBCONSTR}}}}, 52
  \item {\textcolor{blue}    {{\tt{NUCLIDE}}}}, 10

  \indexspace

  \item {\textcolor{blue}    {{\tt{ODD\_ADD\_PM}}}}, 19
  \item {\textcolor{blue}    {{\tt{ODD\_ADD\_TS}}}}, 18
  \item {\textcolor{blue}    {{\tt{ODD\_SCA\_PM}}}}, 18
  \item {\textcolor{blue}    {{\tt{ODD\_SCA\_TS}}}}, 17, 66
  \item {\textcolor{blue}    {{\tt{OMEGA\_RTP}}}}, 50
  \item {\textcolor{blue}    {{\tt{OMEGA\_TURN}}}}, 51
  \item {\textcolor{blue}    {{\tt{OMEGA\_XYZ}}}}, 50, 63
  \item {\textcolor{blue}    {{\tt{OMEGAY}}}}, 50
  \item {\textcolor{blue}    {{\tt{OMISO\_XYZ}}}}, 50
  \item {\textcolor{blue}    {{\tt{OMISOY}}}}, 50
  \item {\textcolor{blue}    {{\tt{ONE\_LINE}}}}, 56
  \item {\textcolor{blue}    {{\tt{OPTI\_GAUSS}}}}, 46, 65, 69

  \indexspace

  \item {\textcolor{blue}    {{\tt{PAIR\_FORCE}}}}, 21
  \item {\textcolor{blue}    {{\tt{PAIR\_INTER}}}}, 21
  \item {\textcolor{blue}    {{\tt{PAIR\_MATRI}}}}, 19, 28
  \item {\textcolor{blue}    {{\tt{PAIRING}}}}, 27
  \item {\textcolor{blue}    {{\tt{PAIRNFORCE}}}}, 20, 21
  \item {\textcolor{blue}    {{\tt{PAIRNINTER}}}}, 21
  \item {\textcolor{blue}    {{\tt{PAIRPFORCE}}}}, 20, 21
  \item {\textcolor{blue}    {{\tt{PAIRPINTER}}}}, 21
  \item {\textcolor{blue}    {{\tt{PARAKERNEL}}}}, 31
  \item {\textcolor{blue}    {{\tt{PARITY}}}}, 25
  \item {\textcolor{blue}    {{\tt{PHASESPACE}}}}, 12, 69, 71
  \item {\textcolor{blue}    {{\tt{PHNONE\_NEU}}}}, 34
  \item {\textcolor{blue}    {{\tt{PHNONE\_PRO}}}}, 34
  \item {\textcolor{blue}    {{\tt{PHPARI\_NEU}}}}, 38
  \item {\textcolor{blue}    {{\tt{PHPARI\_PRO}}}}, 38
  \item {\textcolor{blue}    {{\tt{PHSIGN\_NEU}}}}, 41
  \item {\textcolor{blue}    {{\tt{PHSIGN\_PRO}}}}, 42
  \item {\textcolor{blue}    {{\tt{PHSIMP\_NEU}}}}, 36
  \item {\textcolor{blue}    {{\tt{PHSIMP\_PRO}}}}, 36
  \item {\textcolor{blue}    {{\tt{PING-PONG}}}}, 11
  \item {\textcolor{blue}    {{\tt{PRINT-INTR}}}}, 55
  \item {\textcolor{blue}    {{\tt{PRINT-ITER}}}}, 55
  \item {\textcolor{blue}    {{\tt{PRINT-MOME}}}}, 55
  \item {\textcolor{blue}    {{\tt{PRINT\_AMP}}}}, 56
  \item {\textcolor{blue}    {{\tt{PRINT\_VIOL}}}}, 56
  \item {\textcolor{blue}    {{\tt{PROJECTGCM}}}}, 30, 60

  \indexspace

  \item {\textcolor{blue}    {{\tt{READ\_WOODS}}}}, 63
  \item {\textcolor{blue}    {{\tt{REC\_FIELDS}}}}, 62
  \item {\textcolor{blue}    {{\tt{RECLIPFILE}}}}, 61
  \item {\textcolor{blue}    {{\tt{RECORDFILE}}}}, 58
  \item {\textcolor{blue}    {{\tt{RECORDSAVE}}}}, 59
  \item {\textcolor{blue}    {{\tt{RECYUKFILE}}}}, 61
  \item {\textcolor{blue}    {{\tt{REP\_FIELDS}}}}, 62
  \item {\textcolor{blue}    {{\tt{REPLAYFILE}}}}, 58
  \item {\textcolor{blue}    {{\tt{REPLIPFILE}}}}, 61
  \item {\textcolor{blue}    {{\tt{REPYUKFILE}}}}, 60
  \item {\textcolor{blue}    {{\tt{RESTART}}}}, 63
  \item {\textcolor{blue}    {{\tt{REVIEW}}}}, 58
  \item {\textcolor{blue}    {{\tt{REVIEWFILE}}}}, 58
  \item {\textcolor{blue}    {{\tt{ROTATION}}}}, 25

  \indexspace

  \item {\textcolor{blue}    {{\tt{SAVEKERNEL}}}}, 30, 60
  \item {\textcolor{blue}    {{\tt{SCHIFF\_MOM}}}}, 54
  \item {\textcolor{blue}    {{\tt{SIGNATUREY}}}}, 25
  \item {\textcolor{blue}    {{\tt{SIMPLEXY}}}}, 25
  \item {\textcolor{blue}    {{\tt{SKYRME-SET}}}}, 14
  \item {\textcolor{blue}    {{\tt{SKYRME-STD}}}}, 14, 15, 65
  \item {\textcolor{blue}    {{\tt{SLOW-DOWN}}}}, 45
  \item {\textcolor{blue}    {{\tt{SLOW-PAIR}}}}, 20, 46
  \item {\textcolor{blue}    {{\tt{SLOWLIPKIN}}}}, 33
  \item {\textcolor{blue}    {{\tt{SPICON\_OME}}}}, 51
  \item {\textcolor{blue}    {{\tt{SPICON\_XYZ}}}}, 51
  \item {\textcolor{blue}    {{\tt{SPIN\_ORBIT}}}}, 14, 15
  \item {\textcolor{blue}    {{\tt{SPINCONSTR}}}}, 51
  \item {\textcolor{blue}    {{\tt{SURFAC\_DEF}}}}, 49, 64, 65
  \item {\textcolor{blue}    {{\tt{SURFAC\_PAR}}}}, 48
  \item {\textcolor{blue}    {{\tt{SURFCONSTR}}}}, 53

  \indexspace

  \item {\textcolor{blue}    {{\tt{TIMEREVERS}}}}, 27
  \item {\textcolor{blue}    {{\tt{TRANCUTPRI}}}}, 56
  \item {\textcolor{blue}    {{\tt{TRANSITION}}}}, 31
  \item {\textcolor{blue}    {{\tt{TSIMPLEX3D}}}}, 27
  \item {\textcolor{blue}    {{\tt{TSIMPLEX\_Y}}}}, 27
  \item {\textcolor{blue}    {{\tt{TSIMPLEXES}}}}, 27

  \indexspace

  \item {\textcolor{blue}    {{\tt{VACPAR\_NEU}}}}, 38
  \item {\textcolor{blue}    {{\tt{VACPAR\_PRO}}}}, 38
  \item {\textcolor{blue}    {{\tt{VACSIG\_NEU}}}}, 41
  \item {\textcolor{blue}    {{\tt{VACSIG\_PRO}}}}, 41
  \item {\textcolor{blue}    {{\tt{VACSIM\_NEU}}}}, 36
  \item {\textcolor{blue}    {{\tt{VACSIM\_PRO}}}}, 36

  \indexspace

  \item {\textcolor{blue}    {{\tt{WAVEF\_FILE}}}}, 60
  \item {\textcolor{blue}    {{\tt{WOODSAFILE}}}}, 59

  \indexspace

  \item {\textcolor{blue}    {{\tt{YUKAWASAVE}}}}, 60
  \item {\textcolor{blue}    {{\tt{YUKAWATERM}}}}, 21

\end{theindex}


==> index_of_subjects.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item $K$-mixed states, 56, 68
  \item $K$-mixing, 32
  \item $g$-factor, 66

  \indexspace

  \item acronym, 14, 17, 66
  \item adiabatic, 73, 75, 76
  \item after variation, 15
  \item alignment, 39, 76
  \item AMP (1D), 30
  \item AMP (3D), 30
  \item AMP calculations, 30, 31, 56, 73, 79, 80
  \item AMP energy, 56, 67
  \item AMP kernels, 30, 56
  \item angular frequency, 8, 25, 39, 50, 51, 56, 63, 66, 74--78, 80
  \item angular momentum, 30, 39, 50, 51, 56, 57, 63, 66, 67, 76, 78
  \item angular momentum projection (see AMP), 30
  \item array dimensions, 67, 69
  \item ATLAS BLAS, 70
  \item atomic gas, 10
  \item average neutron pairing gap, 79
  \item average values, 21, 39, 56, 66--68
  \item axial states, 30
  \item axial symmetry, 48, 57, 74

  \indexspace

  \item Basic Linear Algebra Subprogams, 70
  \item BCS equation, 12, 19, 28
  \item BCS pairing, 12, 20, 21, 25, 27, 28, 50
  \item before variation, 15
  \item BLAS, 70, 71
  \item blocking approximation (see diabatic blocking or quasiparticle blocking),
		10
  \item Bohr deformation parameters, 54, 67
  \item broken parity, 25, 66
  \item broken particle-number symmetry, 79
  \item broken signature, 25, 30
  \item broken simplex, 25, 28, 66
  \item broken symmetry, 25, 27, 29, 50, 51, 65, 77, 78
  \item broken time-reversal, 27, 74--76
  \item Broyden method, 46

  \indexspace

  \item canonical state, 13
  \item Cartesian axes, 67
  \item Cartesian components, 50
  \item Cartesian directions, 46, 48, 65, 69, 79
  \item center-of-mass, 14, 15, 65, 66
  \item chaotic, 12, 74
  \item charge block, 12
  \item charge--parity block, 38
  \item charge--parity--signature block, 41
  \item charge--simplex block, 12, 36, 78
  \item collective states, 32
  \item comment, 8, 65, 70, 72
  \item compatibility, 25, 27, 28, 51
  \item compilation, 67
  \item compiler, 70--72
  \item complex hermitian matrices, 71
  \item conserved symmetry, 12, 25--27, 34--42, 44, 45, 54, 57, 65,
		74--76, 78
  \item constant potential, 19
  \item constraint, 45, 50, 51, 53, 54, 67, 74, 77
  \item contact forces, 28
  \item converged solution, 75, 80
  \item convergence, 10, 46, 56, 65, 74, 76
  \item coordinate-space calculations, 79
  \item Coulomb direct energy, 22, 67
  \item Coulomb direct mean field, 22
  \item Coulomb direct potential, 59
  \item Coulomb energy, 64
  \item Coulomb exchange energy, 22, 62, 65, 67
  \item Coulomb exchange mean field, 22
  \item Coulomb file, 59, 60, 74
  \item Coulomb Green function, 45
  \item Coulomb interaction, 79
  \item Coulomb mean field, 45, 59, 64
  \item coupling constants, 14--19, 22, 65, 66
  \item CPU time, 25, 69, 71, 72, 74, 80
  \item cranking term, 50
  \item crossing bands, 75
  \item cutoff energy, 13, 21, 48, 79

  \indexspace

  \item data line, 8, 9, 14, 16, 58--62
  \item data set, 8, 58, 67, 74
  \item data value, 8
  \item default value, 8, 9, 11, 12, 14, 60, 73, 74
  \item deformation, 65, 66, 74, 79
  \item deformation $\gamma $, 56
  \item deformed harmonic oscillator, 48
  \item density matrix, 13, 21, 61, 64
  \item density-dependent part, 17
  \item density-dependent term, 79
  \item diabatic blocking, 12, 34, 37, 39, 40, 42, 73, 74
  \item diabatic-blocking data, 12
  \item diagonalization, 12, 69, 78
  \item direct matrix elements, 22
  \item divergence, 11, 12, 74, 76--78
  \item double precision, 70, 71
  \item doubly-magic nucleus, 78
  \item download, 70, 71

  \indexspace

  \item earlier versions, 28
  \item editor script, 70
  \item eigenstate, 12, 78
  \item eigenstate of Routhian, 35, 37, 40, 42
  \item eigenvalue of HFB mean-field, 56
  \item eigenvectors, 71
  \item electric multipole moment, 54
  \item electric transition, 68
  \item elementary charge, 65
  \item end of input data file, 8
  \item energy, 66
  \item energy density functional, 50, 53
  \item equivalent-spectrum, 79
  \item Euler angles, 29--31, 66
  \item exchange matrix elements, 22
  \item execution, 72
  \item external HO potential, 24

  \indexspace

  \item false-vacuum approximation, 10
  \item Fermi energy, 19, 33, 67, 79
  \item field file, 60--62, 64
  \item filling approximation, 28
  \item first iteration, 19, 29, 46, 63, 64, 66, 78, 79
  \item fixed pairing gap, 28
  \item FORTRAN source, 69, 70
  \item FORTRAN-77, 70
  \item FORTRAN-90, 47, 70, 72

  \indexspace

  \item Gauss-Hermite integration, 46
  \item Gauss-Hermite nodes, 69, 79
  \item Gauss-Hermite quadrature, 65
  \item Gauss-Legendre nodes, 22, 23, 30, 31, 68, 80
  \item Gauss-Tchebyschev nodes, 30, 31, 68, 80
  \item Gaussian-expansion method, 22, 64
  \item GCM kernels, 30
  \item generalized spin-orbit, 14, 15
  \item GOTO BLAS, 70
  \item Green-function method, 22

  \indexspace

  \item Hamiltonian, 56
  \item hardware, 70
  \item Hermite polynomials, 46
  \item HFB calculations, 79
  \item HFB equation, 28
  \item HFB pairing, 13, 19--21, 25, 27, 28, 33, 63
  \item HO basis, 24, 48, 63--65, 69--71, 74, 76, 79
  \item HO quanta, 65, 69
  \item HO state, 48, 69
  \item hole state, 12, 28, 37, 39, 42

  \indexspace

  \item initial mean field, 10, 79
  \item initial rotation, 10
  \item input data, 8, 22, 31, 67, 74, 78--80
  \item input data file, 8, 14, 15, 58, 59, 73, 74, 77--80
  \item input item, 8, 73, 74
  \item input parameter, 8, 60, 69, 73, 74, 78
  \item Intel Math Kernel Library, 70
  \item intrinsic frame, 55, 66, 67, 78
  \item intrinsic spin, 52, 76, 79
  \item item, 8
  \item iteration, 10--12, 22, 39, 44--46, 48, 51, 55, 56, 58--66,
		74--79
  \item iteration number, 11

  \indexspace

  \item Kerman-Onishi condition, 78
  \item kernel, 30, 31, 56, 60, 68
  \item kernel file, 31, 32, 60
  \item keyword line, 8, 9
  \item kinetic energy, 67
  \item kinetic-energy operator, 15

  \indexspace

  \item Landau parameters, 15
  \item LAPACK subroutine, 71
  \item last iteration, 62
  \item linear momentum, 15
  \item link, 71
  \item Lipkin-Nogami file, 61, 64
  \item Lipkin-Nogami method, 32, 61, 64, 73, 80
  \item Lipkin-Nogami parameter, 32, 33, 56
  \item Lipkin-Nogami parameters, 32

  \indexspace

  \item magic numbers, 78
  \item magnetic moment, 45, 55, 67
  \item magnetic transition, 68
  \item mass, 65
  \item mass distribution, 77, 78
  \item matrix elements, 23, 60--62, 64, 79
  \item mean-field Hamiltonian, 12
  \item mean-field Routhian, 35, 37, 40, 42
  \item memory, 31, 44, 69--71
  \item mixing, 20, 46
  \item mixing fraction, 33, 46, 62
  \item moment of inertia, 67
  \item multipole moment, 39, 45, 53, 55, 66

  \indexspace

  \item NAGLIB subroutine, 71
  \item neutron skin, 79
  \item Nilsson asymptotic state, 66
  \item Nilsson labels, 57, 67
  \item Nilsson potential, 10, 48, 64, 74--76, 79
  \item norm eigenvalues, 32, 68
  \item norm kernels, 67, 68
  \item normalization factor, 53
  \item nuclear surface, 48, 65, 74
  \item nucleon mass, 22
  \item number of iterations, 10
  \item number of neutrons, 12

  \indexspace

  \item occupied, 36, 38--41, 67, 76
  \item occupied state, 34, 36, 38, 78
  \item odd nuclei, 10, 25, 57
  \item odd-odd nuclei, 10, 25, 35, 37, 40, 43
  \item one-body center-of-mass, 15
  \item orbital angular momentum, 52
  \item overlap, 35, 37, 40, 42, 44

  \indexspace

  \item pairing, 20, 27, 28, 46, 67, 74--76, 78, 79
  \item pairing energy, 66, 67
  \item pairing force, 20, 21, 28
  \item pairing form-factor, 20, 21, 79
  \item pairing gap, 19, 20, 28, 56, 67, 79
  \item pairing matrix elements, 28
  \item pairing strength, 19, 28
  \item pairing window, 12, 13, 79
  \item parallel calculations, 80
  \item parameter set, 14
  \item parity, 38--42, 44, 45, 66, 74--78
  \item parity block, 38, 40, 67, 77, 78
  \item parity symmetry, 25
  \item parity--signa\discretionary {-}{}{}ture configuration, 28
  \item parity--signature block, 28, 41, 42, 66, 67, 76, 77
  \item parity--signature configuration, 29, 42, 78
  \item particle number, 10, 30
  \item particle state, 12, 28, 37, 39, 42
  \item particle-hole channel, 46
  \item particle-hole configuration, 12, 66
  \item particle-hole excitation, 34, 36, 38, 39, 41, 78
  \item particle-number symmetry, 79
  \item particle-particle channel, 79
  \item Pauli exclusion principle, 34, 36, 38
  \item phase space, 10
  \item ping-pong, 11, 12, 74, 76, 77
  \item pion mass, 22
  \item planar solution, 76, 78
  \item principal axes, 49
  \item principal-axes frame, 66

  \indexspace

  \item quadrupole moment, 39, 66, 74, 77, 79
  \item quasiparticle blocking, 10, 35, 37, 40, 42, 44
  \item quasiparticle energy, 55
  \item quasiparticle properties, 55
  \item quasiparticle state, 21, 69, 79

  \indexspace

  \item radius, 66
  \item rearrangement energy, 67
  \item recommended value, 12, 73, 74
  \item record file, 44, 58, 59, 62, 63
  \item reduced kernels, 56, 68
  \item reduced matrix elements, 31, 56, 68
  \item reference configuration, 34, 36, 38, 41
  \item replay file, 58, 63
  \item restored symmetry, 25
  \item review file, 58
  \item root-mean-square radii, 79
  \item rotating state, 35, 79
  \item Routhian, 40, 55, 56, 66, 67, 75, 76

  \indexspace

  \item saturation density, 20, 79
  \item scalar constraint, 54
  \item scalar multipole moment, 54
  \item Schiff moment, 31, 54, 56
  \item security measure, 29, 31
  \item self-consistent mean field, 22, 24
  \item self-consistent solution, 11, 78
  \item seniority pairing force, 28
  \item short-range correction, 22
  \item signature, 30, 41, 42, 44, 74--76
  \item signature symmetry, 25, 29
  \item simplex, 25, 27, 36, 37, 74--76, 78
  \item simplex block, 37, 66, 67
  \item simplex symmetry, 29
  \item Simpson integration, 45
  \item single-particle configuration, 34, 75, 77
  \item single-particle energy, 10, 67
  \item single-particle observables, 12
  \item single-particle properties, 55, 58
  \item single-particle state, 36, 66, 69
  \item Skyrme force, 14--16, 65
  \item Skyrme functional, 10, 16, 65, 66
  \item Skyrme parameter set, 16, 18
  \item Slater approximation, 22
  \item solid harmonics, 45
  \item space inversion, 29
  \item spatial coordinates, 79
  \item spherical basis, 78, 79
  \item spherical code, 79
  \item spherical ground state, 78, 79
  \item spherical harmonics, 53
  \item spherical HO basis, 29, 30
  \item spin, 39, 51, 66, 67
  \item spin-orbit, 14, 67
  \item stability, 10, 11, 67
  \item stability energy, 46, 66
  \item standard FORTRAN input, 8
  \item standard FORTRAN output, 65
  \item starting point, 79
  \item state-dependent pairing gaps, 28
  \item subroutine, 70--72
  \item sum rules, 56, 68
  \item Sun Performance Library, 70
  \item superdeformed, 8, 73, 74
  \item surface multipole moment, 45, 53--55
  \item switches, 67
  \item symmetry axis, 57
  \item symmetry-violating terms, 56

  \indexspace

  \item tensor, 14
  \item termination of the HF iteration, 10
  \item theorem about self-consistent symmetries, 78
  \item tilted-axis cranking, 73, 76
  \item time-even contribution, 66, 67
  \item time-even coupling constants, 16--18
  \item time-even potential, 46
  \item time-odd contribution, 66, 67
  \item time-odd coupling constants, 15, 17--19
  \item time-odd potential, 46
  \item time-reversal symmetry, 25, 27, 29, 74, 76
  \item time-reversed partner, 35, 37, 40, 42
  \item traditional spin-orbit, 14
  \item transition electric moment, 31, 56
  \item transition magnetic moment, 31, 56
  \item transition surface moment, 31, 56
  \item triaxial deformation, 76--80
  \item two-body center-of-mass, 15

  \indexspace

  \item vector machine, 69
  \item vector processor, 69

  \indexspace

  \item wave function, 12, 29, 31, 44, 59, 60
  \item wave function file, 60
  \item Wigner function, 30
  \item Woods-Saxon file, 59, 63
  \item work flow, 68

  \indexspace

  \item Yukawa calculations, 60, 61
  \item Yukawa fields, 64
  \item Yukawa file, 60, 61, 64
  \item Yukawa interaction, 22

  \indexspace

  \item zero-range density-dependent interaction, 79
  \item zero-range density-dependent pairing, 20, 21

\end{theindex}


==> index_of_subroutines.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item {\textcolor{green}    {{\tt{CGEMM}}}}, 71, 72
  \item {\textcolor{green}    {{\tt{CPU\_TIME}}}}, 72
  \item {\textcolor{green}    {{\tt{CPUTIM}}}}, 72

  \indexspace

  \item {\textcolor{green}    {{\tt{DCLOCK}}}}, 72
  \item {\textcolor{green}    {{\tt{DSMALG}}}}, 30

  \indexspace

  \item {\textcolor{green}    {{\tt{ETIME}}}}, 72

  \indexspace

  \item {\textcolor{green}    {{\tt{F02AXE}}}}, 71, 72

  \indexspace

  \item {\textcolor{green}    {{\tt{GETTIM}}}}, 72

  \indexspace

  \item {\textcolor{green}    {{\tt{PARAMS}}}}, 14
  \item {\textcolor{green}    {{\tt{PREDEF}}}}, 8

  \indexspace

  \item {\textcolor{green}    {{\tt{REVIEW}}}}, 58

  \indexspace

  \item {\textcolor{green}    {{\tt{SETBAS}}}}, 65

  \indexspace

  \item {\textcolor{green}    {{\tt{TIME}}}}, 72

  \indexspace

  \item {\textcolor{green}    {{\tt{ZGECO}}}}, 72
  \item {\textcolor{green}    {{\tt{ZGEDI}}}}, 72
  \item {\textcolor{green}    {{\tt{ZHEEVR}}}}, 71
  \item {\textcolor{green}    {{\tt{ZHPEV}}}}, 71, 72
  \item {\textcolor{green}    {{\tt{ZHPEVX}}}}, 71, 72

\end{theindex}

